A Comparison between RSMA, SDMA, and OMA in Multibeam LEO Satellite Systems

Low Earth orbit (LEO) satellite systems enable close to global coverage and are therefore expected to become important pillars of future communication standards. However, a particular challenge faced by LEO satellites is the high orbital velocities due to which a precise channel estimation is difficult. We model this influence as an erroneous angle of departure (AoD), which corresponds to imperfect channel state information (CSI) at the transmitter (CSIT). Poor CSIT and non-orthogonal user channels degrade the performance of space-division multiple access (SDMA) precoding by increasing inter-user interference (IUI). In contrast to SDMA, there is no IUI in orthogonal multiple access (OMA), but it requires orthogonal time or frequency resources for each user. Rate-splitting multiple access (RSMA), unifying SDMA, OMA, and non-orthogonal multiple access (NOMA), has recently been proven to be a flexible approach for robust interference management considering imperfect CSIT. In this paper, we investigate RSMA as a promising strategy to manage IUI in LEO satellite downlink systems caused by non-orthogonal user channels as well as imperfect CSIT. We evaluate the optimal configuration of RSMA depending on the geometrical constellation between the satellite and users.

==> Paper-WSA(1)/figures/RS.tex <==

\begin{tikzpicture}
	\node[draw,minimum height=0.5cm,minimum width=3cm,rotate=90,align=center,color={rgb:red,0;green,0.4470;yellow,0.7410}] at (4, -2.25) (d)  {Linear Precoder};
	
	\node[draw,minimum height=0.5cm,minimum width=3cm,rotate=90,align=center] at (2.75, -2.25) (enc)  {Encoder};
	
	\node[draw,minimum height=0.5cm,minimum width=1.75cm,rotate=90,align=center] at (1.35, -1.65) (mes)  {Message\\ Combiner};
	
	\node[draw,minimum height=0.3cm,minimum width=3cm,rotate=90,align=center] at (-0.4, -2.25) (splitter)  {Message Splitter};
	
	\node[draw,minimum height=0.5cm,minimum width=3cm,rotate=90,align=center] at (-2, -2.25) (data)  {User Data};

	\draw[decoration={markings,mark=at position 1 with
	{\arrow[scale=2,>=stealth]{>}}},postaction={decorate}]	(-1.75, -1)--(-0.75, -1) node[midway,below,yshift=0.025cm,xshift=-0.1cm] {\small$ {{B}}_{1}$} node[midway, below,yshift=-0.35cm] {$\vdots$};
    \draw[decoration={markings,mark=at position 1 with
	{\arrow[scale=2,>=stealth]{>}}},postaction={decorate}]	(-1.75, -2.25)--(-0.75, -2.25) node[midway,below,yshift=0.025cm,xshift=-0.1cm] {\small$ {{B}}_{k}$} node[midway, below,yshift=-0.35cm] {$\vdots$};
	\draw[decoration={markings,mark=at position 1 with
		{\arrow[scale=2,>=stealth]{>}}},postaction={decorate}]	(-1.75, -3.5)--(-0.75, -3.5) node[midway,below,yshift=0.025cm,xshift=-0.1cm] {\small$ {{B}}_{K}$};
	
	\draw[decoration={markings,mark=at position 1 with
		{\arrow[scale=2,>=stealth]{>}}},postaction={decorate}]	(-0.1, -1)--(0.8, -1) node[midway,below,yshift=0.025cm,xshift=0.1cm] {\small$ {{B}}_{c,1}$};
	\draw[decoration={markings,mark=at position 1 with
		{\arrow[scale=2,>=stealth]{>}}},postaction={decorate}]	(-0.1, -1.55)--(0.8, -1.55) node[midway,below,yshift=0.025cm,xshift=0.1cm] {\small$ {{B}}_{c,k}$} node[near start,above,yshift=-0.05cm,xshift=-0.09cm] {{\fontsize{2}{6} $\vdots$}};
	\draw[decoration={markings,mark=at position 1 with
		{\arrow[scale=2,>=stealth]{>}}},postaction={decorate}]	(-0.1, -2.1)--(0.8, -2.1) node[midway,below,yshift=0.025cm,xshift=0.1cm] {\small$ {{B}}_{c,K}$} node[near start,above,yshift=-0.05cm,xshift=-0.09cm] {{\fontsize{2}{6} $\vdots$}};
	
	    \draw[decoration={markings,mark=at position 1 with
		{\arrow[scale=2,>=stealth]{>}}},postaction={decorate}]	(1.9, -1.5)--(2.5, -1.5) node[midway,below,yshift=0.025cm] {\small$ {{B}}_c$};
		\draw[decoration={markings,mark=at position 1 with
		{\arrow[scale=2,>=stealth]{>}}},postaction={decorate}]	(3, -1.5)--(3.75, -1.5) node[midway,below,yshift=0.025cm] {\small$ {{s}}_c$};

	
		\draw[decoration={markings,mark=at position 1 with
		{\arrow[scale=2,>=stealth]{>}}},postaction={decorate}]	(-0.1, -2.7)--(2.5, -2.7) node[midway,below,yshift=0.025cm,xshift=0.05cm] {\small$ {{B}}_{p,1}$};
	\draw[decoration={markings,mark=at position 1 with
		{\arrow[scale=2,>=stealth]{>}}},postaction={decorate}]	(-0.1, -3.2)--(2.5, -3.2) node[midway,below,yshift=0.025cm,xshift=0.05cm] {\small$ {{B}}_{p,k}$} node[near start,above,yshift=-0.05cm,xshift=-0.5cm] {{\fontsize{2}{6} $\vdots$}};
	\draw[decoration={markings,mark=at position 1 with
		{\arrow[scale=2,>=stealth]{>}}},postaction={decorate}]	(-0.1, -3.7)--(2.5, -3.7) node[midway,below,yshift=0.025cm,xshift=0.05cm] {\small$ {{B}}_{p,K}$} node[near start,above,yshift=-0.05cm,xshift=-0.5cm] {{\fontsize{2}{6} $\vdots$}};
	
	
	\draw[decoration={markings,mark=at position 1 with
		{\arrow[scale=2,>=stealth]{>}}},postaction={decorate}]	(3, -2.7)--(3.74, -2.7) node[midway,below,yshift=0.025cm,xshift=0.05cm] {\small$ {{s}}_1$};
	\draw[decoration={markings,mark=at position 1 with
		{\arrow[scale=2,>=stealth]{>}}},postaction={decorate}]	(3, -3.2)--(3.74, -3.2) node[midway,below,yshift=0.025cm,xshift=0.05cm] {\small$ {{s}}_k$} node[near start,above,yshift=-0.05cm,xshift=-0.075cm] {{\fontsize{2}{6} $\vdots$}};
	\draw[decoration={markings,mark=at position 1 with
		{\arrow[scale=2,>=stealth]{>}}},postaction={decorate}]	(3, -3.7)--(3.74, -3.7) node[midway,below,yshift=0.025cm,xshift=0.05cm] {\small$ {{s}}_K$} node[near start,above,yshift=-0.05cm,xshift=-0.075cm] {{\fontsize{2}{6} $\vdots$}};
		
	\draw[decoration={markings,mark=at position 1 with
		{\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (4.25,-1) -- (5,-1)  node[midway, below] {${x}_1$} node[midway, below,yshift=-0.35cm] {$\vdots$};
	\draw[decoration={markings,mark=at position 1 with
		{\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (4.25,-2.25) -- (5,-2.25)  node[midway, below] {${x}_n$} node[midway, below,yshift=-0.35cm] {$\vdots$};
	\draw[decoration={markings,mark=at position 1 with
		{\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (4.25,-3.5) -- (5,-3.5)  node[midway, below] {${x}_N$};
	
	
	%\node[draw,dashed,minimum height=3.5cm,minimum width=5.6cm,align=center] at (1.85, -2.25) { };

	
\end{tikzpicture}

==> Paper-WSA(1)/figures/correlation.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}

\begin{axis}[%
width=5.677in,
height=1.519in,
at={(0.952in,0.531in)},
scale only axis,
xmin=0,
xmax=200,
xlabel style={font=\color{white!15!black}},
xlabel style={font=\fontsize{18pt}{20}\selectfont},
xlabel={User Distance $D_k$ [km]},
ymin=0,
ymax=1,
ytick={  0, 0.5,   1},
ylabel style={font=\color{white!15!black}},
ylabel style={font=\fontsize{18pt}{20}\selectfont},
ylabel={$\rho$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids
]
\addplot [color=mycolor1, line width=2pt, forget plot, mark=square, mark options={solid, mycolor1},mark repeat=50,mark phase=25,mark size=3pt]
  table[row sep=crcr]{%
0.5	0.999990004776705\\
1	0.999960019550714\\
1.5	0.999910045608974\\
2	0.99984008519423\\
2.5	0.999750141276004\\
3	0.99964021790274\\
3.5	0.999510319778929\\
4	0.999360452649053\\
4.5	0.999190623020435\\
5	0.999000838375682\\
5.5	0.998791106955043\\
6	0.998561437998445\\
6.5	0.998311841476811\\
7	0.998042328399735\\
7.5	0.997752910389571\\
8	0.99744360029914\\
8.5	0.997114411380802\\
9	0.996765358317625\\
9.5	0.996396456024542\\
10	0.99600772097023\\
10.5	0.995599169850515\\
11	0.99517082063168\\
11.5	0.994722692021032\\
12	0.994254803637245\\
12.5	0.99376717562189\\
13	0.993259829589585\\
13.5	0.992732787293394\\
14	0.992186071964917\\
14.5	0.991619707480597\\
15	0.991033718541024\\
15.5	0.990428130500269\\
16	0.98980296973844\\
16.5	0.989158263516144\\
17	0.988494040052075\\
17.5	0.987810327978091\\
18	0.98710715719302\\
18.5	0.986384558408639\\
19	0.985642562666154\\
19.5	0.984881202619919\\
20	0.984100511170778\\
20.5	0.983300522022944\\
21	0.982481270221124\\
21.5	0.981642790984782\\
22	0.98078512111053\\
22.5	0.979908297162592\\
23	0.979012357870726\\
23.5	0.978097341751826\\
24	0.977163288257755\\
24.5	0.976210237895686\\
25	0.975238231979469\\
25.5	0.974247312309627\\
26	0.9732375219626\\
26.5	0.972208904494468\\
27	0.971161504305036\\
27.5	0.970095366413297\\
28	0.969010537308476\\
28.5	0.967907063227928\\
29	0.966784991882584\\
29.5	0.965644372139143\\
30	0.964485251918604\\
30.5	0.963307681875235\\
31	0.96211171257417\\
31.5	0.960897395006608\\
32	0.95966478210433\\
32.5	0.95841392597656\\
33	0.957144880615352\\
33.5	0.955857700410366\\
34	0.954552440586267\\
34.5	0.953229156745806\\
35	0.951887905366523\\
35.5	0.950528744671589\\
36	0.949151731506646\\
36.5	0.94775692518282\\
37	0.946344385463522\\
37.5	0.944914172763237\\
38	0.943466347112463\\
38.5	0.942000970798341\\
39	0.940518105883095\\
39.5	0.939017815597346\\
40	0.937500163806207\\
40.5	0.935965214222526\\
41	0.934413032409424\\
41.5	0.93284368487865\\
42	0.93125723626674\\
42.5	0.929653755307862\\
43	0.928033309606069\\
43.5	0.926395966803436\\
44	0.924741796232117\\
44.5	0.923070868017164\\
45	0.921383252279404\\
45.5	0.919679020243877\\
46	0.917958243399827\\
46.5	0.916220994350372\\
47	0.914467346242023\\
47.5	0.912697371520687\\
48	0.910911145404001\\
48.5	0.90910874234016\\
49	0.907290237052598\\
49.5	0.905455707249019\\
50	0.903605227486553\\
50.5	0.901738876792426\\
51	0.899856731441288\\
51.5	0.897958870275723\\
52	0.896045372456542\\
52.5	0.89411631735449\\
53	0.892171785097849\\
53.5	0.890211856451408\\
54	0.888236611881615\\
54.5	0.886246134006095\\
55	0.884240504432167\\
55.5	0.882219806501666\\
56	0.880184121884469\\
56.5	0.878133536881521\\
57	0.876068134413466\\
57.5	0.873987999873689\\
58	0.871893218634648\\
58.5	0.869783875742133\\
59	0.867660059334135\\
59.5	0.865521853964773\\
60	0.863369349222206\\
60.5	0.861202631260979\\
61	0.85902178990116\\
61.5	0.856826912718117\\
62	0.854618089995307\\
62.5	0.852395410234592\\
63	0.850158964847686\\
63.5	0.847908843926209\\
64	0.845645137920427\\
64.5	0.843367938979328\\
65	0.841077339997247\\
65.5	0.838773430296238\\
66	0.836456306351095\\
66.5	0.834126058500487\\
67	0.831782782005884\\
67.5	0.829426569597388\\
68	0.827057516548449\\
68.5	0.824675716845124\\
69	0.822281266341109\\
69.5	0.819874260223033\\
70	0.817454794321691\\
70.5	0.815022965206329\\
71	0.81257886794348\\
71.5	0.810122601018408\\
72	0.807654262364487\\
72.5	0.805173948240411\\
73	0.802681756161631\\
73.5	0.800177784854597\\
74	0.797662133151277\\
74.5	0.795134900886698\\
75	0.792596185603038\\
75.5	0.790046087393991\\
76	0.787484705671019\\
76.5	0.78491214095122\\
77	0.782328494468932\\
77.5	0.779733865132693\\
78	0.777128354937249\\
78.5	0.774512064709497\\
79	0.771885095232236\\
79.5	0.76924754995299\\
80	0.766599528589255\\
80.5	0.7639411344777\\
81	0.761272470724121\\
81.5	0.758593637584754\\
82	0.755904739573067\\
82.5	0.7532058798014\\
83	0.75049716064527\\
83.5	0.747778686614593\\
84	0.745050560756895\\
84.5	0.742312886465925\\
85	0.739565767937059\\
85.5	0.736809309079803\\
86	0.734043615849313\\
86.5	0.731268789834877\\
87	0.72848493930677\\
87.5	0.725692165694547\\
88	0.722890575688532\\
88.5	0.720080274539737\\
89	0.717261366474645\\
89.5	0.714433957014833\\
90	0.711598151430538\\
90.5	0.708754056691353\\
91	0.705901776558702\\
91.5	0.703041418541836\\
92	0.700173087206772\\
92.5	0.697296889749542\\
93	0.694412931051555\\
93.5	0.691521316844315\\
94	0.68862215442205\\
94.5	0.685715550413841\\
95	0.6828016098141\\
95.5	0.679880439378601\\
96	0.676952146368223\\
96.5	0.674016836650875\\
97	0.671074615265722\\
97.5	0.668125590942881\\
98	0.665169868913334\\
98.5	0.662207556809548\\
99	0.659238759766896\\
99.5	0.656263586026004\\
100	0.653282139756377\\
100.5	0.650294529280231\\
101	0.647300860834002\\
101.5	0.644301240613062\\
102	0.641295775889373\\
102.5	0.638284571557729\\
103	0.63526773643873\\
103.5	0.632245374840954\\
104	0.629217592947998\\
104.5	0.626184498257912\\
105	0.623146197349712\\
105.5	0.620102794513142\\
106	0.617054397699062\\
106.5	0.614001111495205\\
107	0.610943041981327\\
107.5	0.607880296345791\\
108	0.604812979171226\\
108.5	0.601741196264833\\
109	0.598665052984357\\
109.5	0.595584656030916\\
110	0.592500108967346\\
110.5	0.589411516969248\\
111	0.586318986924202\\
111.5	0.583222622598178\\
112	0.580122528739028\\
112.5	0.577018810085143\\
113	0.573911571705425\\
113.5	0.570800916997356\\
114	0.567686950629158\\
114.5	0.564569776908899\\
115	0.561449499472787\\
115.5	0.558326222721178\\
116	0.555200047718383\\
116.5	0.55207108241911\\
117	0.548939425684784\\
117.5	0.545805181199736\\
118	0.542668454529825\\
118.5	0.539529344400972\\
119	0.5363879564995\\
119.5	0.53324439068736\\
120	0.530098750900886\\
120.5	0.526951135601544\\
121	0.523801649861415\\
121.5	0.52065039301579\\
122	0.517497467190246\\
122.5	0.514342971923655\\
123	0.511187008236767\\
123.5	0.508029677331579\\
124	0.504871078801681\\
124.5	0.501711310882636\\
125	0.498550474558823\\
125.5	0.495388668838538\\
126	0.492225993855211\\
126.5	0.489062545952662\\
127	0.485898424184164\\
127.5	0.482733729227149\\
128	0.479568555545913\\
128.5	0.476403002460254\\
129	0.473237167398287\\
129.5	0.470071146403968\\
130	0.46690503659181\\
130.5	0.463738934681814\\
131	0.460572935291195\\
131.5	0.457407136405659\\
132	0.45424163140392\\
132.5	0.451076516705057\\
133	0.447911885722875\\
133.5	0.444747835098681\\
134	0.441584457188158\\
134.5	0.438421844717225\\
135	0.43526009336583\\
135.5	0.432099295042752\\
136	0.428939542289264\\
136.5	0.425780928336855\\
137	0.422623544026242\\
137.5	0.419467482189049\\
138	0.416312833113076\\
138.5	0.413159687951751\\
139	0.410008137455534\\
139.5	0.406858271454469\\
140	0.403710179896862\\
140.5	0.400563951686503\\
141	0.397419677835789\\
141.5	0.394277443912577\\
142	0.391137340192028\\
142.5	0.387999453927574\\
143	0.384863872276061\\
143.5	0.381730682299876\\
144	0.378599971470908\\
144.5	0.375471825567865\\
145	0.372346329043953\\
145.5	0.369223569649398\\
146	0.366103630966663\\
146.5	0.362986596782633\\
147	0.359872553326591\\
147.5	0.356761582754599\\
148	0.353653769309689\\
148.5	0.350549195843102\\
149	0.347447942368341\\
149.5	0.344350094993437\\
150	0.341255731928325\\
150.5	0.338164936494211\\
151	0.33507778713825\\
151.5	0.331994366351386\\
152	0.328914752145821\\
152.5	0.325839024771401\\
153	0.322767263701297\\
153.5	0.319699545736332\\
154	0.316635950523272\\
154.5	0.313576555019209\\
155	0.310521436672271\\
155.5	0.307470670061518\\
156	0.304424333513135\\
156.5	0.301382502827191\\
157	0.298345251875699\\
157.5	0.295312656245506\\
158	0.292284789840574\\
158.5	0.28926172583598\\
159	0.286243539618197\\
159.5	0.28323030287516\\
160	0.280222086874068\\
160.5	0.277218965736606\\
161	0.27422100858046\\
161.5	0.271228288634666\\
162	0.268240874167399\\
162.5	0.265258835868006\\
163	0.262282244844306\\
163.5	0.259311167907819\\
164	0.256345674477943\\
164.5	0.253385831930186\\
165	0.250431710107074\\
165.5	0.247483372839027\\
166	0.244540889574233\\
166.5	0.241604324895343\\
167	0.238673742793236\\
167.5	0.235749211157455\\
168	0.232830792852576\\
168.5	0.22991855262681\\
169	0.227012554639428\\
169.5	0.224112860094963\\
170	0.221219532451576\\
170.5	0.21833263358329\\
171	0.215452225079643\\
171.5	0.212578369990937\\
172	0.209711125186138\\
172.5	0.206850552883157\\
173	0.203996713350842\\
173.5	0.201149662534705\\
174	0.198309462419873\\
174.5	0.195476169090265\\
175	0.192649840094764\\
175.5	0.189830532851534\\
176	0.187018304146434\\
176.5	0.184213208757807\\
177	0.181415302899166\\
177.5	0.178624640834239\\
178	0.175841278147095\\
178.5	0.173065267968662\\
179	0.170296663247298\\
179.5	0.167535518783627\\
180	0.164781885020638\\
180.5	0.16203581324661\\
181	0.159297356636255\\
181.5	0.156566564573055\\
182	0.153843488967537\\
182.5	0.151128178940183\\
183	0.148420683002131\\
183.5	0.145721051406908\\
184	0.143029329721318\\
184.5	0.140345567387584\\
185	0.137669812451043\\
185.5	0.135002110768927\\
186	0.132342508589325\\
186.5	0.129691051658745\\
187	0.127047783237997\\
187.5	0.124412752470572\\
188	0.121785999359898\\
188.5	0.119167569144623\\
189	0.116557504270458\\
189.5	0.113955848397577\\
190	0.111362643128516\\
190.5	0.108777930775729\\
191	0.10620175094532\\
191.5	0.103634144296485\\
192	0.101075151687316\\
192.5	0.098524813530974\\
193	0.0959831672768957\\
193.5	0.0934502521772679\\
194	0.0909261059542236\\
194.5	0.088410766552102\\
195	0.0859042716317815\\
195.5	0.0834066561009322\\
196	0.0809179564854526\\
196.5	0.0784382091609082\\
197	0.075967448906355\\
197.5	0.0735057094218447\\
198	0.0710530256952007\\
198.5	0.0686094301878988\\
199	0.0661749575836394\\
199.5	0.0637496382419673\\
200	0.0613335058404119\\
};
\end{axis}


\end{tikzpicture}%

==> Paper-WSA(1)/figures/verteilteSatellitenplus.tex <==

\begin{tikzpicture}
	
	%	\begin{pgfonlayer}[Ebene2]	
	\coordinate (center) at (3,3);
	\coordinate (2) at (3, 5);
	\coordinate (3) at ($(center) +(80:4)$);%22.5
	\coordinate (4) at ($(center) +(120:4)$);%157.25
	\coordinate (5) at (3,6.99);
	\coordinate (6) at ($(center) +(75:2)$);
	\coordinate (7) at ($(center) +(130:2)$);
	%\coordinate (userk) at (1.9,4.7)
	%\coordinate (userkl) at (1.4,4.25)
	\coordinate (8) at ($(center) +(0:0.3)$);
	\coordinate (9) at ($(center) +(89:0.3)$);
	\coordinate (10) at ($(center) +(0:0.75)$);
	\coordinate (11) at ($(center) +(142:0.75)$);
	
	\coordinate (12) at ($(3,4.25) +(91:0.3)$);
	\coordinate (13) at ($(3,4.25) +(269:0.3)$);
	
	\coordinate (14) at ($(1.4,4.25) +(0:0.6)$);
	\coordinate (15) at ($(1.4,4.25) +(60:0.6)$);
	
	\coordinate (16) at ($(5) +(180:0.95)$);
	\coordinate (17) at ($(5) +(245:0.95)$);
	
	\coordinate (18) at ($(5) +(180:0.4)$);
	\coordinate (19) at ($(5) +(269:0.4)$);

	\draw[black,dotted]
	let \p1 = ($(3) - (center)$),
	\p2 = ($(4) - (center)$),
	\n0 = {veclen(\x1,\y1)},            % Radius
	\n1 = {atan(\y1/\x1)+180*(\x1<0)},  % initial angle
	\n2 = {atan(\y2/\x2)+180*(\x2<0)}   % Final angle
	in
	(3) arc(\n1:\n2:\n0)   ;
	
	\draw[black,dotted]
	let \p1 = ($(6) - (center)$),
	\p2 = ($(7) - (center)$),
	\n0 = {veclen(\x1,\y1)},            % Radius
	\n1 = {atan(\y1/\x1)+180*(\x1<0)},  % initial angle
	\n2 = {atan(\y2/\x2)+180*(\x2<0)}   % Final angle
	in
	(6) arc(\n1:\n2:\n0) ;
	
	
\draw[black,decoration={markings,mark=at position 1 with
	{\arrow[scale=1,>=stealth]{>}}},postaction={decorate}]
let \p1 = ($(18) - (5)$),
\p2 = ($(19) - (5)$),
\n0 = {veclen(\x1,\y1)},            % Radius
\n1 = {atan(\y1/\x1)+180*(\x1<0)},  % initial angle
\n2 = {atan(\y2/\x2)+180*(\x2<0)}   % Final angle
in
(18) arc(\n1:\n2:\n0) node[near start,xshift=0.185cm,yshift=-0.05cm] { \tiny$ {\theta}_{k}$} ;

\filldraw[draw=black,opacity=0.2, fill={rgb:red,0;green,0.4470;yellow,0.7410}, fill opacity=0.1]
let \p1 = ($(18) - (5)$),
\p2 = ($(19) - (5)$),
\n0 = {veclen(\x1,\y1)},            % Radius
\n1 = {atan(\y1/\x1)+180*(\x1<0)},  % initial angle
\n2 = {atan(\y2/\x2)+180*(\x2<0)}   % Final angle
in
(5) --  (18) arc(\n1:\n2:\n0)   -- cycle;

\draw[black,decoration={markings,mark=at position 1 with
	{\arrow[scale=1,>=stealth]{>}}},postaction={decorate}]
let \p1 = ($(16) - (5)$),
\p2 = ($(17) - (5)$),
\n0 = {veclen(\x1,\y1)},            % Radius
\n1 = {atan(\y1/\x1)+180*(\x1<0)},  % initial angle
\n2 = {atan(\y2/\x2)+180*(\x2<0)}   % Final angle
in
(16) arc(\n1:\n2:\n0) node[near start,xshift=0.41cm,yshift=-0.2cm] { \tiny$ {\theta}_{k-1}$} ;

\filldraw[draw=black,opacity=0.2, fill={rgb:red,0;green,0.4470;yellow,0.7410}, fill opacity=0.1]
let \p1 = ($(16) - (5)$),
\p2 = ($(17) - (5)$),
\n0 = {veclen(\x1,\y1)},            % Radius
\n1 = {atan(\y1/\x1)+180*(\x1<0)},  % initial angle
\n2 = {atan(\y2/\x2)+180*(\x2<0)}   % Final angle
in
(5) --  (16) arc(\n1:\n2:\n0)   -- cycle;
	

	\draw[dotted,color={rgb:red,0;green,0.4470;yellow,0.7410},decoration={markings,mark=at position 1 with
		{\arrow[scale=1,>=stealth]{>}}},postaction={decorate}] (3,6.9) -- (3,5.25) node[midway,xshift=0.08cm,yshift=-0.25cm,left] {\tiny $\mathbf{h}_k$};
	\draw[dotted,color={rgb:red,0;green,0.4470;yellow,0.7410},decoration={markings,mark=at position 1 with
		{\arrow[scale=1,>=stealth]{>}}},postaction={decorate}] (3,6.9) -- (2,4.95) node[midway,xshift=-0.08cm,yshift=-0.16cm,left] {\tiny $\mathbf{h}_{k-1}$};	

	
		\draw[decoration={markings,mark=at position 1 with
		{\arrow[scale=1.25,>=stealth]{|}}},postaction={decorate}] (3.5,6) -- (3.5,5.1) node[at start,xshift=-0.05cm,yshift=-0.1cm,right] {\tiny $d_0$};
	
		\draw[decoration={markings,mark=at position 1 with
		{\arrow[scale=1.25,>=stealth]{|}}},postaction={decorate}] (3.5,6) -- (3.5,6.9);
	
	\node[black] (UE1) at (3.1,4.92) {\tiny$ k$};
	\node[black] (UE2) at (1.65,4.6) {\tiny$ k-1$};

	
	\draw[draw = black,opacity = 1,decoration={markings,mark=at position 1 with
	{\arrow[scale=1,>=stealth]{|}}},postaction={decorate}] (2.6,4.625) -- (2.1,4.5) node[at start,below,xshift=0.15cm,yshift=-0.03cm] {\tiny \color{black} $D_k$};
	\draw[draw = black,opacity = 1,decoration={markings,mark=at position 1 with {\arrow[scale=1,>=stealth]{|}}},postaction={decorate}] (2.6,4.625) -- (3.1,4.75) node[at start,above,xshift=0.05cm,yshift=-0.03cm] {\tiny \color{black} };
	
	\begin{pgfonlayer}{background} 
		\node[inner sep=0.1pt] (russell) at (3,6.88)
		{\includegraphics[width=0.1\linewidth]{figures/sat}};
	\end{pgfonlayer}


	\begin{pgfonlayer}{background}
		\node[opacity =1,inner sep=0.1pt] (russell) at (2,4.75)
		{\includegraphics[width=0.025\linewidth]{figures/user_klein}};
	\end{pgfonlayer}
	\begin{pgfonlayer}{background}
		\node[opacity =1,inner sep=0.1pt] (russell) at (3,5.05)
		{\includegraphics[width=0.025\linewidth]{figures/user_klein}};
	\end{pgfonlayer}

\end{tikzpicture}


==> Paper-WSA(1)/my_lib/acronyms.tex <==
\begin{acronym}
	%\acro{tx}[AP]{acces point}
	\acro{rx}[GS]{ground station}
	\acro{dl}[DL]{downlink}
	\acro{mimo}[MIMO]{multiple-input-multiple-output}
	\acro{ntn}[NTN]{non-terrestrial network}
	\acro{geo}[GEO]{geostationary orbit}
	\acro{meo}[MEO]{medium Earth orbit}
	\acro{leo}[LEO]{low Earth orbit}
	\acro{qos}[QoS]{quality of service}
	\acro{dip}[DiP]{distributed precoding}
	\acro{pspc}[PAPPC]{per-acces point power constraint}
	\acro{kkt}[KKT]{Karush-Kuhn-Tucker}
	\acro{svd}[SVD]{singular value decomposition}
	\acro{mse}[MSE]{mean-squared error}
	\acro{mmse}[MMSE]{minimum mean-squared error}
	\acro{zf}[ZF]{zero-forcing}
	\acro{mrt}[MRT]{maximum ratio transmission}
	\acro{mrc}[MRC]{maximum ratio combining}
	\acro{snr}[SNR]{signal-to-noise ratio}
	\acro{sinr}[SINR]{signal-to-interference-and-noise ratio}
	\acro{sic}[SIC]{successive interference cancellation}
	\acro{csi}[CSI]{channel state information}
	\acro{csit}[CSIT]{\ac{csi} at the transmitter}
	\acro{csir}[CSIR]{\ac{csi} at the receiver}
	\acro{los}[LOS]{line-of-sight}
	\acro{aod}[AoD]{angle of departure}
	\acro{aoa}[AoA]{angle of arrival}
	\acro{ula}[ULA]{uniform linear array}
	\acro{ecef}[ECEF]{Earth-centered, Earth-fixed }
	\acro{dft}[DFT]{discrete Fourier transform}
	\acro{sota}[SotA]{state of the art}
	\acro{rsma}[RSMA]{rate-splitting multiple access}
	\acro{sdma}[SDMA]{space-division multiple access}
	\acro{oma}[OMA]{orthogonal multiple access}
	\acro{noma}[NOMA]{non-orthogonal multiple access}
    \acro{tdma}[TDMA]{time-division multiple access}
    \acro{ofdma}[OFDMA]{orthogonal frequency-division multiple access}
	\acro{awgn}[AWGN]{additive white Gaussian noise}
	\acro{iui}[IUI]{inter-user interference}
	\acro{3gpp}[3GPP]{3rd Generation Partnership Project}
\end{acronym}


==> Paper-WSA(1)/my_lib/mathsymbols.tex <==
\usepackage{amssymb}
\def\mathbi#1{\textbf{\em #1}}  % to use the command mathbi{}

\newcommand{\vek}[1]{\ensuremath{\mathbf{#1}}}          % vector
\newcommand{\vekt}[1]{\ensuremath{\tilde{\vek{#1}}}}        % modified vector
\newcommand{\vekhat}[1]{\ensuremath{\hat{\vek{#1}}}}        % estimated vector

\newcommand{\Lagrange}{\ensuremath{\boldsymbol{\Lambda}}}          % vector
\newcommand{\lagrange}{\ensuremath{\boldsymbol{\lambda}}}          % vector
\newcommand{\lagranget}{\ensuremath{\tilde{\boldsymbol{\lambda}}}}          % vector
\newcommand{\lagrangee}{\ensuremath{\boldsymbol{\nu}}}          % vector

%\newcommand{\eigmtx}{\ensuremath{\boldsymbol{\Xi}}}
%\newcommand{\eigmin}{\ensuremath{\xi_{min}}}
%\newcommand{\eigmax}{\ensuremath{\xi_{max}}}

\newcommand{\Exvl}[1]{\ensuremath{\mathrm{E}\left\{#1\right\}}}
\newcommand{\var}[1]{\ensuremath{\mathrm{Var}\left\{#1\right\}}}
%\newcommand{\err}{\ensuremath{\vek{E}}}
%\newcommand{\ChErr}{\ensuremath{\boldsymbol{\Xi}}}
\newcommand{\nvar}{\ensuremath{\sigma_\mathsf{n}^2}}
\newcommand{\naltvar}{\bar{\sigma}_{\mathsf{n}}^2}
\newcommand{\Naltvar}{\bar{\boldsymbol{\Sigma}}_{\mathsf{n}}^2}

\newcommand{\itk}{\ensuremath{^{(k)}}}          
\newcommand{\itkp}{\ensuremath{^{(k+1)}}}       

\newcommand{\NS}{\ensuremath{N_{\text{S}}}}          % vector
\newcommand{\NU}{\ensuremath{N_{\text{U}}}}
\newcommand{\Nt}{\ensuremath{N_{\text{t}}}}
\newcommand{\Nr}{\ensuremath{N_{\text{r}}}}
\newcommand{\NTx}{\ensuremath{N_{\text{Tx}}}}
\newcommand{\NRx}{\ensuremath{N_{\text{Rx}}}}
\newcommand{\NI}{\ensuremath{N_{\text{I}}}}
\newcommand{\NO}{\ensuremath{N_{\text{O}}}}
\newcommand{\NE}{\ensuremath{|\mathcal{E}|}}
\newcommand{\Lf}{\ensuremath{L}}
\newcommand{\NIt}{\ensuremath{N_{\text{It}}}}

\newcommand{\GTx}{\ensuremath{\zeta_{\text{Tx,dB}}}}
\newcommand{\GRx}{\ensuremath{\zeta_{\text{Rx,dB}}}}

\newcommand{\DA}{\ensuremath{D_{\text{A}}}}
\newcommand{\DS}{\ensuremath{D_{\text{S}}}}

\newcommand{\Ptx}{\ensuremath{P_{\text{Tx}}}}

\newcommand{\aoa}{\ensuremath{\theta}}
\newcommand{\aoal}{\ensuremath{\theta_\ell}}
\newcommand{\aod}{\ensuremath{\Theta}}
\newcommand{\aodl}{\ensuremath{\Theta_\ell}}

\newcommand{\estaoa}{\ensuremath{\aoa_{\ell,\text{est}}}}
\newcommand{\erraoa}{\ensuremath{\varepsilon}}
\newcommand{\erraoamtx}{\ensuremath{\vek{E}}}
\newcommand{\estaod}{\ensuremath{\aod_{\ell,\text{est}}}}
\newcommand{\erraod}{\ensuremath{\tilde{\varepsilon}}}
\newcommand{\erraodmtx}{\ensuremath{\vekt{E}}}



\newcommand{\RE}{\ensuremath{r_{\text{E}}}}

\newcommand{\Graph}{\ensuremath{\mathcal{G}}}
\newcommand{\Lagr}{\ensuremath{\mathcal{L}}}
\newcommand{\J}{\ensuremath{\mathcal{J}}}
\newcommand{\V}{\ensuremath{\mathcal{V}}}
\newcommand{\N}{\ensuremath{\mathcal{N}}}
\newcommand{\E}{\ensuremath{\mathcal{E}}}
\renewcommand{\H}{\ensuremath{\mathrm{H}}}
\newcommand{\T}{\ensuremath{\mathrm{T}}}

\newcommand{\C}{\ensuremath{\mathbb{C}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}

\newcommand{\A}{\ensuremath{\mathbb{A}}}
\newcommand{\FLOPS}{\ensuremath{\mathcal{F}}}
\newcommand{\Symbols}{\ensuremath{\mathcal{S}}}
\newcommand{\D}{\ensuremath{\text{D}}}
\newcommand{\PtP}{\ensuremath{\text{P2P}}}
\newcommand{\PtMP}{\ensuremath{\text{P2MP}}}

\newcommand{\fc}{\ensuremath{f_{\text{c}}}}

\newcommand{\veka}{\ensuremath{\vek{a}}}
\newcommand{\vekb}{\ensuremath{\vek{b}}}
\newcommand{\vekx}{\ensuremath{\vek{x}}}
\newcommand{\veks}{\ensuremath{\vek{s}}}
\newcommand{\veksest}{\ensuremath{\vekt{s}}}
\newcommand{\vekv}{\ensuremath{\vek{v}}}
\newcommand{\veky}{\ensuremath{\vek{y}}}
\newcommand{\vekz}{\ensuremath{\vek{z}}}
\newcommand{\vekc}{\ensuremath{\vek{c}}}
\newcommand{\vekp}{\ensuremath{\vek{p}}}
\newcommand{\vekn}{\ensuremath{\vek{n}}}

\newcommand{\vekta}{\ensuremath{\vekt{a}}}
\newcommand{\vektv}{\ensuremath{\vekt{v}}}
\newcommand{\vektx}{\ensuremath{\vekt{x}}}
\newcommand{\vekhatx}{\ensuremath{\vekhat{x}}}
\newcommand{\vektz}{\ensuremath{\vekt{z}}}
\newcommand{\vekhatz}{\ensuremath{\vekhat{z}}}

\newcommand{\EQ}{\ensuremath{\vek{W}}}
\newcommand{\eq}{\ensuremath{\vek{w}}}
\newcommand{\eqsat}{\ensuremath{\vek{w}_{\ell}}}
\newcommand{\PC}{\ensuremath{\vek{G}}}
\newcommand{\pc}{\ensuremath{\vek{g}}}
\newcommand{\pcsat}{\ensuremath{\vek{g}_{\ell}}}
\newcommand{\vekgi}{\ensuremath{\vek{g}_i}}
\newcommand{\vekg}{\ensuremath{\vek{g}}}


\newcommand{\vekH}{\ensuremath{\vek{H}}}
\newcommand{\vekHH}{\ensuremath{\vek{H}\vek{H}^H}}
%\newcommand{\vekHeff}{\ensuremath{\vek{H}_{\text{eff}}}}
%\newcommand{\vekHest}{\ensuremath{\vekhat{H}}}
\newcommand{\vekHerr}{\ensuremath{\vekt{H}}}
\newcommand{\vekHsat}{\ensuremath{\vek{H}_{\ell}}}
\newcommand{\vekh}{\ensuremath{\vek{h}}}

\newcommand{\chrx}[1]{\ensuremath{\underbar{\vekh}_{#1}}}
\newcommand{\chtx}[1]{\ensuremath{\vekH_{#1}}}
\newcommand{\cheff}{\ensuremath{\vek{H}_{\text{eff}}}}
\newcommand{\chest}{\ensuremath{\vekt{H}}}

\newcommand{\vekC}{\ensuremath{\vek{C}}}
\newcommand{\vekI}{\ensuremath{\vek{I}}}
\newcommand{\vekT}{\ensuremath{\vek{T}}}
\newcommand{\vekS}{\ensuremath{\vek{S}}}
\newcommand{\vekM}{\ensuremath{\vek{M}}}
\newcommand{\vekW}{\ensuremath{\vek{W}}}
\newcommand{\vekF}{\ensuremath{\vek{F}}}
\newcommand{\vekR}{\ensuremath{\vek{R}}}
\newcommand{\vekr}{\ensuremath{\vek{r}}}
\newcommand{\vekd}{\ensuremath{\vek{d}}}
\newcommand{\vekP}{\ensuremath{\vek{P}}}

\newcommand{\vekD}{\ensuremath{\vek{D}}}
\newcommand{\vekL}{\ensuremath{\vek{L}}}
\newcommand{\vekU}{\ensuremath{\vek{U}}}
\newcommand{\vekV}{\ensuremath{\vek{V}}}
\newcommand{\vekSig}{\ensuremath{\boldsymbol{\Sigma}}}
\newcommand{\vekA}{\ensuremath{\vek{A}}}
\newcommand{\vekB}{\ensuremath{\vek{B}}}

\newcommand{\source}{\mathbi{x}}

\newcommand{\sinr}{\ensuremath{\text{SINR}}}
%\newcommand{\EbN0}{\ensuremath{\frac{\bar{E}_b}{N_0}}}
\newcommand{\dB}{\ensuremath{\text{dB}}}   
\newcommand{\real}[1]{\ensuremath{\operatorname{Re}\left\{#1\right\}}} 
\newcommand{\imag}[1]{\ensuremath{\operatorname{Im}\left\{#1\right\}}} 
\newcommand{\diag}[1]{\ensuremath{\operatorname{diag}\left(#1\right)}}
\newcommand{\blkdiag}[1]{\ensuremath{\operatorname{blkdiag}\left(#1\right)}}
\newcommand{\tr}[1]{\ensuremath{\operatorname{tr}\left\{#1\right\}}} 
\newcommand{\rank}[1]{\ensuremath{\operatorname{rank}\left(#1\right)}}
\newcommand{\sinc}[1]{\ensuremath{\operatorname{sinc}\left(#1\right)}} 

\newcommand{\vekxj}{\ensuremath{\vek{x}_{j}}}
\newcommand{\vekxjk}{\ensuremath{\vek{x}_{j}^{(k)}}}
\newcommand{\vekxjkp}{\ensuremath{\vek{x}_{j}^{(k+1)}}}
\newcommand{\vekxjkm}{\ensuremath{\vek{x}_{j}^{(k-1)}}}
\newcommand{\vekxik}{\ensuremath{\vek{x}_{i}^{(k)}}}
\newcommand{\vekxikp}{\ensuremath{\vek{x}_{i}^{(k+1)}}}
\newcommand{\vekxikm}{\ensuremath{\vek{x}_{i}^{(k-1)}}}
\newcommand{\covx}{\ensuremath{\vek{C}_\vekx}}

\newcommand{\nullvec}{\boldsymbol{0}}   % (fette) Vektoren oder Matrizen (jeder einzeln...)
%\newcommand{\avec}{\mathbf{a}}
%\newcommand{\Avec}{\mathbf{A}}
%\newcommand{\bvec}{\mathbf{b}}
%\newcommand{\Bvec}{\mathbf{B}}
%\newcommand{\cvec}{\mathbf{c}}
%\newcommand{\Cvec}{\mathbf{C}}
%\newcommand{\dvec}{\mathbf{d}}
%\newcommand{\Dvec}{\mathbf{D}}
%\newcommand{\evec}{\mathbf{e}}
%\newcommand{\Evec}{\mathbf{E}}
%\newcommand{\fvec}{\mathbf{f}}
%\newcommand{\Fvec}{\mathbf{F}}
%\newcommand{\gvec}{\mathbf{g}}
%\newcommand{\Gvec}{\mathbf{G}}
%\newcommand{\hvec}{\mathbf{h}}
%\newcommand{\Hvec}{\mathbf{H}}
%\newcommand{\ivec}{\mathbf{i}}
%\newcommand{\Ivec}{\mathbf{I}}
%\newcommand{\lvec}{\mathrm{\mathbf $\ell$}}
%\newcommand{\Mvec}{\mathbf{M}}
%\newcommand{\Nvec}{\mathbf{N}}
%\newcommand{\Pvec}{\mathbf{P}}
%\newcommand{\Qvec}{\mathbf{Q}}
%\newcommand{\rvec}{\mathbf{r}}
%\newcommand{\Rvec}{\mathbf{R}}
%\newcommand{\svec}{\mathbf{s}}
%\newcommand{\Svec}{\mathbf{S}}
%\newcommand{\Tvec}{\mathbf{T}}
%\newcommand{\uvec}{\mathbf{u}}
%\newcommand{\Uvec}{\mathbf{U}}
%\newcommand{\vvec}{\mathbf{v}}
%\newcommand{\Vvec}{\mathbf{V}}
%\newcommand{\wvec}{\mathbf{w}}
%\newcommand{\Wvec}{\mathbf{W}}
%\newcommand{\xvec}{\mathbf{x}}
%\newcommand{\Xvec}{\mathbf{X}}
%\newcommand{\yvec}{\mathbf{y}}
%\newcommand{\Yvec}{\mathbf{Y}}
%\newcommand{\zvec}{\mathbf{z}}
%\newcommand{\Zvec}{\mathbf{Z}}


